High-accuracy mesh-free quadrature for trimmed parametric surfaces and volumes

This work presents a high-accuracy, mesh-free, generalized Stokes theorem-based numerical quadrature scheme for integrating functions over trimmed parametric surfaces and volumes. The algorithm relies on two fundamental steps: (1) We iteratively reduce the dimensionality of integration using the generalized Stokes theorem to line integrals over trimming curves, and (2) we employ numerical antidifferentiation in the generalized Stokes theorem using high-order quadrature rules. The scheme achieves exponential convergence up to trimming curve approximation error and has applications to computation of geometric moments, immersogeometric analysis, conservative field transfer between high-order curvilinear meshes, and initialization of multi-material simulations. We compare the quadrature scheme to commonly-used quadrature schemes in the literature and show that our scheme is much more efficient in terms of number of quadrature points used. We provide an open-source implementation of the scheme in MATLAB as part of QuaHOG, a software package for Quadrature of High-Order Geometries.

==> section02_computingRationalMoments.tex <==
\section{Numerical Integration over Rational Regions}
\label{sec:algorithm}

We first consider a genus-zero planar region $\Omega$ with a closed, connected, oriented boundary loop $\Gamma$ such that the normal to $\Gamma$ points toward the interior of the region $\Omega$. 
%
We take the boundary loop $\Gamma$ to be composed of $n_c$ rational oriented component curves $\{\mathbf{c}_i\}_{i=1}^{n_c}$, where the $\mathbf{c}_{i}$ are given in the rational Bernstein-\bezier\ basis:

\begin{equation*}
  \mathbf{c}_i(s) = 
    \begin{cases} x_i(s) = \frac{\displaystyle\sum_{j=0}^{m_i} w_{i,j} x_{i,j} B^{m_i}_j(s)}{\displaystyle\sum_{j=0}^{m_i} w_{i,j} B^{m_i}_j(s)} \\
                  y_i(s) =  \frac{\displaystyle\sum_{j=0}^{m_i} w_{i,j} y_{i,j} B^{m_i}_j(s)}{\displaystyle\sum_{j=0}^{m_i} w_{i,j} B^{m_i}_j(s)}
    \end{cases} 
    1 \leq i \leq n_c,
\end{equation*}
   for $0\leq s \leq 1$ such that $\Gamma = \cup_{i=1}^{n_c} \mathbf{c}_i$, where $m_i$ are the degrees of the component curves, $w_{i,j}$ are the control weights, and $x_{i,j},y_{i,j}$ are the control points.  The Bernstein-\bezier\ basis is defined as 
  \begin{equation}
  B_j^m(s) = {m\choose{j}} (1-s)^{j}s^{m-j},
  \end{equation} and has a multitude of useful properties~\cite{farin2002curves,farouki2012}. For rational curves, the control weight matrix $w_{i,j}$ has at least one entry such that $w_{i,j} \neq 1$ for some $i,j$. We denote the maximum degree of the component curves as $m= \max_{i \leq n_c} (m_i)$.
%
\begin{figure}
  \centering
  \includegraphics[width=.8\linewidth]{wrench}
  \caption{
    A wrench-shaped region bounded by rational curves over which polynomials can be integrated to machine precision using the \spectralPE\ algorithm. 
    This example illustrates the object's first few geometric moments, as computed by the \spectralPE\ algorithm:
    The grey area represents its area (0$^{th}$ moment), 
    the black dot represents its centroid (1$^{st}$ moment), 
    and the ellipse represents its moment of inertia (2$^{nd}$ moment). }
  \label{fig:example_region}
\end{figure}
%
We denote the bounding box of the control points of the region $\Omega$ as
\begin{equation*}
\tilde{\Omega} = [\min_{i,j}\{x_{i,j}\}, \max_{i,j}\{x_{i,j}\} ] \times [\min_{i,j}\{y_{i,j}\}, \max_{i,j}\{y_{i,j}\} ].
\end{equation*} 

Both the \spectral\ and \spectralPE\ algorithms compute quadrature points $\{(x_l,y_l)\}_{l=1}^{n_q}$ and weights $\{w_l\}_{l=1}^{n_q}$ such that the error
\begin{equation*}
E = \left|\iint _{\Omega} f(x,y) dx dy - \sum_{l=1}^{n_q} w_l f(x_l,y_l)\right| < \mathcal{O}(e^{-cn_q}),
\end{equation*}  
decreases exponentially with respect to number of quadrature points for some constant $c$ for smooth integrands in the bounding box of $\Omega$, $f(x,y) \in \mathcal{C}^\infty(\tilde{\Omega})$,
where $n_q$ is the number of quadrature points. This is because they are based on one-dimensional high-order quadrature rules, which can be shown to have exponential convergence (c.f. \cite{davis2007methods}).
%
If the function has only $k$ continuous derivatives,  $f(x,y) \in \mathcal{C}^k (\tilde{\Omega})$, then the scheme attains the maximum algebraic order of convergence possible, $E = \mathcal{O}(n_q^{-k+1})$.

Moreover, because it uses rational quadrature for the intermediate quadrature rule, the \spectralPE\ quadrature rule is exact up to machine precision, $\epsilon$, for polynomials $p(x,y)$ of maximal degree $k$ or less with an \textit{a priori} known number of quadrature points $n_q$, which, as we derive in Section~$\ref{sec:modification}$, is:
\begin{equation}
	n_q = \left\lceil{\frac{k+1}{2}}\right\rceil\sum_{i=1}^{n_c} \left(m_i(k + 3)+1\right).
\end{equation}

%
%
Figure~\ref{fig:example_region} shows an example of a wrench-shaped region composed of $n_c=46$~component curves, all of which are rational and of degree $m_i=3$.
%
The \spectralPE\ quadrature scheme requires $n_q = 1472$ quadrature points to exactly integrate polynomials up to degree $k=2$ and $n_q = 1748$ quadrature points to exactly integrate polynomials up to degree $k=3$. This works out to $32$ and $38$ quadrature points per component curve, respectively, for $k=2$ and $k=3$.
%
Note that the \spectralPE\ quadrature scheme still retains the spectral convergence property for arbitrary smooth integrands, so fewer quadrature points could be used if machine precision is not necessary.

It is important here to emphasize the limitation that the integrand $f(x,y)$ must be smoothly extendable to the bounding box $\tilde{\Omega}$ of the integration region $\Omega$. This is trivially possible when the integrand is polynomial, and is also possible in immersed finite element methods such as immersogeometric analysis and the finite cell method. In these methods, the integrand is defined on a background cell, and the bounding box of the integration region is contained within this background cell. An example is the pink cell in Figure~\ref{fig:immersogeometric_example}. In cases when the integrand cannot be smoothly extended, moment-fitting can be used with the \spectralPE\ algorithm to produce high-order quadrature rules with quadrature points within the domain of integration. We briefly describe moment fitting in~\ref{app:momentFitting}.
%

The general idea behind the present algorithms is to use Green's theorem to transform the integral over the interior region $\Omega$ into a sum of line integrals along each curve $\mathbf{c}_i$,

\begin{align}
\iint_\Omega f(x,y) dxdy &= \int_{\partial \Omega} A_f(x,y) dx \nonumber \\
&= \sum_{i=1}^{n_c} \int_{\mathbf{c}_i} A_f(x,y) dx, \label{eq:green}
\end{align}
where $A_f(x,y)$ is the $y$-antiderivative of the integrand.

The algorithms are overviewed graphically in Figure~\ref{fig:overview} and, for each component curve $\mathbf{c}_i$, can both be summarized in two basic steps:
\begin{enumerate}[(1)]
  \item Compute a set of intermediate quadrature points and weights for the Green's Theorem line integral corresponding to the particular curve $\mathbf{c}_i$, and
  \item Compute quadrature rules to evaluate the antiderivative function numerically at each intermediate quadrature point.
\end{enumerate}
The two quadrature rules' weights are then combined in a tensor-product fashion to produce the quadrature weights for each of the final quadrature points. The \spectral\ and \spectralPE\ algorithms only differ in  the implementation for the first step in the above two-step process. We describe the \spectral\ algorithm initially, then describe how the \spectralPE\ algorithm differs.
%

\subsection{Intermediate Quadrature Rule}
\label{sec:intermediate}
The first step in the algorithm is to convert the area integral inside the domain $\Omega$ into line integrals along each of the curves, $\{\mathbf{c}_{i}\}_{i=1}^{n_c}$, and to find appropriate intermediate quadrature rules for each of these line integrals. 
%
For the purposes of this section, we assume that the antiderivative function
\begin{equation}
A_f(x,y) = \int_{C}^y f(x,t)dt, \label{eq:antiderivative}
\end{equation} 
can be evaluated to high precision at any $(x,y)$ point on any of the component curves $\mathbf{c}_i$. 
We explain our approach for this in the next section (Section~\ref{sec:antiderivative}).

Because the curves are given parametrically, the physical space integrals appearing on the right-hand side of Equation~$\eqref{eq:green}$ can be transformed into the parametric space of each component curve:
\begin{equation}
\int_{\mathbf{c}_i} A_f(x,y) dx = \int_0^1 A_f(x_i(s),y_i(s)) \frac{d x_i(s)}{ds} ds. \label{eq:green_par}
\end{equation}
Each of these integrals can be evaluated using a high-order 1D quadrature scheme, such as Gaussian quadrature with $Q_i$-points, which yields a set of $Q_i$ quadrature points $\{s_{i,q}\}_{q=1}^{Q_i}$ and weights $\{\gamma_{i,q}\}_{q=1}^{Q_i}$. The intermediate quadrature points in $\mathbb{R}^2$ can then be calculated as $(x_{i,q},y_{i,q})= \left(x_i(s_{i,q}),y_i(s_{i,q})\right)$ for each $q=1,\ldots Q_i$. This evaluation can be performed stably for rational Bernstein-\bezier\ curves using de Casteljau's algorithm \cite{farin2002curves}.
%

The intermediate quadrature rule then reads as
\begin{equation}
\iint _{\Omega} f(x,y) dx dy \approx \sum_{i=1}^{n_c} \sum_{q=1}^{Q_i} \gamma_{i,q} A_f(x_{i,q},y_{i,q}) \frac{d x_{i}}{ds}(s_{i,q}). \label{eq:intermediate}
\end{equation}
%

The resulting integrand in each of the line integrals is composed of two parts, one which requires evaluation of the integrand's antiderivative and one which requires evaluation of the derivative of a \bezier\ curve. Derivatives of rational or polynomial \bezier\ curves can be efficiently and stably computed to machine precision using de Casteljau's algorithm. As long as the antiderivative is evaluated to high enough precision, the intermediate quadrature rule will converge exponentially fast as $Q_i$ increases \cite{davis2007methods}.  
%

Next, we describe how to evaluate the antiderivative.

\subsection{Antiderivative Quadrature Rule}
\label{sec:antiderivative}

A key ingredient in the evaluation of the interior function of the intermediate quadrature rule in Equation~$\eqref{eq:intermediate}$ is the evaluation of the antiderivative. A high-order quadrature rule, such as Gaussian quadrature with $P$ points, can be used to evaluate the integrand with spectral convergence as $P$ is increased~\cite{davis2007methods}. In our implementation, for simplicity, we set $P=Q_i$. Note that for some integrands, such as polynomial integrands, the antiderivative can alternatively be evaluated symbolically, which could garner computational efficiency benefits.

The antiderivative quadrature rule will then have quadrature points 
$\{x_{i,q}, y_{i,q,\zeta}\}_{\zeta=1}^{P}$, and weights $\{\gamma_{i,q,\zeta}\}_{\zeta=1}^{P}$. For a particular curve $\mathbf{c}_i$ and intermediate quadrature point $(x_{i,q},y_{i,q})$, the antiderivative can be evaluated as 
\begin{equation}
A_f(x_{i,q},y_{i,q}) = \int_{C}^{y_{i,q}} f(x_{i,q},y) dy \approx \sum_{\zeta=1}^{P} \gamma_{i,q,\zeta}\ f(x_{i,q},y_{i,q,\zeta}). \label{eq:num_antiderivative}
\end{equation}
Note that the $x_{i,q}$ do not depend on the index $\zeta$, since the antiderivative is only with respect to $y$. If the function $f(x,y)$ is a polynomial of degree $k$, then Equation~$\eqref{eq:num_antiderivative}$ will be exact (up to machine precision) with $P= \lceil{\frac{k+1}{2}\rceil}$ points. If the function is smooth, then convergence to the correct integral will be spectral with respect to the number of quadrature points as $P$ is increased.

Although the arbitrary integration constant $C$ in the calculation of $A_f(x,y)$ has no bearing on the validity of Equation~$\eqref{eq:green}$, it can affect the locations and weights of the resulting quadrature scheme as well as the floating point stability, if it chosen to be very far away from the integration domain. We choose $C$ according to the strategy described in ~Section~\ref{sec:green_implement}. 

\subsection{Full Quadrature Rule}
Finally, the intermediate quadrature rule and the numerical antiderivative quadrature rule can be combined to obtain a spectral full quadrature scheme:
\begin{equation}
\iint _{\Omega} f(x,y) dx dy \approx \sum_{i=1}^{n_c} \sum_{q=1}^{Q_i} \sum_{\zeta=1}^{P}  w_{i,q,\zeta} f(x_{i,q},y_{i,q,\zeta}) ,
\end{equation}
where $w_{i,q,\zeta} = \gamma_{i,q} \gamma_{i,q,\zeta} \frac{d x_{i}}{ds}(s_{i,q})$. The derivative terms $\frac{dx_{i}}{ds}$ can be computed efficiently using de Casteljau's algorithm and can be viewed as geometric correction terms to the component Gaussian quadrature weights. The total number of quadrature points used in the final quadrature rule will scale with the number of quadrature points used in each component quadrature rule, $n_q = P\sum_{i=1}^{n_c} Q_i$. If we use $P=Q_i$ and all $Q_i$ equal, then the number of quadrature points will be $n_q = n_c P^2$.

\subsection{A Modified Algorithm for Polynomial Exactness} %-- \spectralPE\ algorithm}
\label{sec:modification}
In some situations, such as calculation of geometric moments and moment-fitting techniques, it is of particular importance to efficiently calculate integrals of polynomial functions over arbitrary rational regions. Calculating these integrals exactly with an \textit{a priori} number of quadrature points can remove the need for potentially expensive adaptive quadrature that attempts to converge to the solution through successively increased number of quadrature points. With a modification to the intermediate quadrature step of the \spectral\ algorithm presented above, we can achieve exactness up to machine precision for polynomial integrands over these regions. We call this quadrature scheme \spectralPE\ (spectral, polynomially exact). Exactness can be achieved by guaranteeing that the two components steps of intermediate quadrature and antiderivative quadrature are exact.

The antiderivative quadrature rule is already exact for polynomial integrands $f(x,y)$ up to a pre-specified degree $k$ if Gaussian quadrature is used with $P=\lceil{\frac{k+1}{2}\rceil}$ points. The intermediate quadrature rule, on the other hand, has no guarantees of exactness for polynomial integrands if Gaussian quadrature is used, since both the antiderivative function $A_f(x(s),y(s))$ and the parametric derivative term $\frac{dx}{ds}$ are rational, rather than polynomial, functions. However, a rational quadrature rule exact for an appropriate class of intermediate rational functions can be used for the intermediate quadrature rule in order to achieve polynomial exactness (up to machine precision). See \ref{app:detailed_example} for a worked-out example of the \spectralPE\ algorithm on a circular domain.
 
\subsubsection{Review of Rational Quadrature}
 Exact quadrature formulas for particular classes of functions such as polynomials have been studied for centuries. Quadrature rules which are exact for polynomials are generally formulated in terms of classes of orthogonal polynomials~\cite{gautschi1999orthogonal}. Two of the most commonly used quadrature rules are Gaussian quadrature and Fej\'er (i.e. Clenshaw-Curtis) quadrature, which are based on the orthogonal Legendre and Chebyshev polynomials, respectively. Exact quadrature formulas for classes of nonpolynomial functions have also been studied in the literature, and are typically based on generalizations of the classical orthogonal polynomials. The first study of orthogonal rational functions was made by Djirbashian in the 1960's, a review of which can be found in~\cite{djrbashian1990survey}. A connection to exact Gauss-type quadrature rules for rational functions with known real poles was first made by Gautschi~\cite{gautschi1993Gauss}. 

More recently, Bultheel, Deckers, and Van Deun have published a series of papers with very efficient algorithms for computing Fej\'er-type quadrature rules exact for rational functions with known poles outside the unit interval in linear time with respect to the total number of poles of the rational functions for which exactness is guaranteed~\cite{deckers2008rational, van2008algorithm, deckers2009computing, deckers2017algorithm}. The algorithm only requires knowing the locations and multiplicities of the poles of the rational functions of interest. 

Next, we describe an algorithm which computes locations and multiplicities of the poles of the rational functions which must be integrated exactly in order to achieve polynomial exactness.


\subsubsection{Poles of Intermediate Rational Functions}
\label{subsec:poles}
For a particular curve $\mathbf{c}_i$, the intermediate rational function which must be integrated exactly is the one that arises as the product of the antiderivative function $A_f(x_i(s))$ and the derivative term $\frac{dx(s)}{ds}$, as seen in Equation~$\eqref{eq:green_par}$. As we shall prove, the poles of the intermediate rational function $A_f(x_i(s)) \frac{dx(s)}{ds}$ do not in fact depend on the function $f(x,y)$ but only on its polynomial degree $k$. In fact, the poles of the intermediate rational function are simply the poles of the original curve $\mathbf{c}_i$ but with the multiplicity of each pole multiplied by $k+3$. To prove this, consider the two terms in the product separately. For clarity, we call $\{p_{i,j}\}_{j=1}^{m_i}$ the poles of the curve $\mathbf{c}_i$, defined as the zeros of the weight function 
\begin{equation*}
w_i(s) =\displaystyle\sum_{j=0}^{m_i} w_{i,j} B^{m_i}_j(s).
\end{equation*}

By the quotient rule, the derivative of a rational function has the effect of doubling the multiplicity of each of its poles. Therefore, $\frac{d x_i(s)}{ds}$ will have the same poles $\{p_{i,j}\}_{j=1}^{m_i}$ as $x_i(s)$, but each will have multiplicity of $2$. 

Since $x_i(s)$ and $y_i(s)$ are each rational functions with poles $\{p_{i,j}\}_{j=1}^{m_i}$ and $A_f(x,y)$ is a polynomial, $A_f(x(s),y(s))$ will also have the poles $\{p_{i,j}\}_{j=1}^{m_i}$. However, each pole's multiplicity will be $k+1$ times as large as the multiplicity it had for $x_i(s)$ or $y_i(s)$. Assuming that $f(x,y)$ is a degree $k$ polynomial and, expressing it in the monomial basis as $f(x,y) = \sum_{k_x+k_y\leq k} a_{k_x,k_y} x^{k_x} y^{k_y}$ for some coefficients $a_{k_x,k_y}$, then 
\begin{equation*}
\resizebox{.99\linewidth}{!}{\parbox{\linewidth}{
\begin{align*}
&A_f(x_i(s),y_i(s)) = \sum_{k_x+k_y\leq k} a'_{k_x,k_y} x_i(s)^{k_x} y_i(s)^{k_y+1} \\
&\hspace{-3mm}= \sum_{k_x+k_y \leq k} \left(a'_{k_x,k_y} \left(\frac{\sum_{j=0}^{m_i} w_{i,j}x_{i,j}B^{m_i}_j(s)}{\sum_{j=0}^{m_i} w_{i,j} B^{m_i}_j(s)}\right)^{k_x} \left(\frac{\sum_{j=0}^{m_i} w_{i,j}y_{i,j}s^j}{\sum_{j=0}^{m_i} w_{i,j} B^{m_i}_j(s)}\right)^{k_y+1} \right)\\
&\hspace{-3mm}= \sum_{k_x+k_y \leq k} \left(a'_{k_x,k_y}\frac{\left(\sum_{j=0}^{m_i} w_{i,j}x_{i,j}B^{m_i}_j(s)\right)^{k_x} \left(\sum_{j=0}^{m_i} w_{i,j}y_{i,j}B^{m_i}_j(s)\right)^{k_y+1}}{\left(\sum_{j=0}^{m_i} w_{i,j} B^{m_i}_j(s)\right)^{k_x+k_y+1}} \right),
\end{align*}
}}
\end{equation*}
where $a'_{k_x,k_y}=a_{k_x,k_y}/(k_y+1)$ and $k_x + k_y$ attains its maximum value of $k$, since $f(x,y)$ is a degree $k$ polynomial.

Combining the above statements, the integrand $A_f(x(s),y(s)) \frac{d x(s)}{d s}$ in Equation~$\eqref{eq:green}$ will have the same poles as the component curves did, namely $\{p_{i,j}\}_{j=1}^{m_i}$. However, each of these poles will have a multiplicity of $k+3$, where $k+1$ of them come from the antiderivative calculation and $2$ of them come from the derivative term. 

Therefore, in order to find a rational intermediate quadrature rule exact for rational functions with the required poles, we must compute the set of poles $\{p_{i,j}\}_{j=1}^{m_i}$ of each component curve $\{\mathbf{c}_i\}_{i=1}^{n_c}$. Because the rational curves are given in terms of control points and control weights, the poles of the rational curves $\{\mathbf{c}_i\}_{i=1}^{n_c}$ can be easily calculated as the roots of the corresponding control weight (i.e. denominator) polynomial, $w_i(s)=\sum_{j=0}^{m_i} w_{i,j} B^{m_i}_j(s)$.

There is a wide body of literature on stable univariate polynomial complex root finding. The roots of a polynomial in the monomial basis can be found by computing the eigenvalues of the polynomial's companion matrix, $A_i$ \cite{edelman1995polynomial}. By converting the polynomial $w_i(s)$ to the monomial basis $w_i(s) = \sum_{j=0}^{m_i} a_{i,j} s^j$ (see ~Section~\ref{sec:conversion}), the companion matrix can be written as 
\begin{align*}
A_i = \begin{bmatrix}
1 & 0 & 0 & \ldots & -\frac{a_{i,1}}{a_{i,m_i}}\\
1 & 1 & 0 & \ldots & -\frac{a_{i,2}}{a_{i,m_i}} \\
0 & 1 & 1 & \ldots & -\frac{a_{i,3}}{a_{i,m_i}} \\
\vdots & \vdots & \vdots & \ddots & \vdots \\
0 & 0 & 0 & \ldots & -1.
\end{bmatrix}
\end{align*}
The eigenvalues of $A_i$ are the roots of $w_i(s)$. Computing the eigenvalues of this $(m_i+1)\times (m_i+1)$ matrix is generally an $\mathcal{O}(m_i^3)$ operation. Finding the roots for all of the rational component curves therefore scales as $\mathcal{O}\left(n_c m^3\right)$ with the maximum degree of the component rational curves $m=\max_{i\leq n_c} (m_i)$, since finding the roots of the control weight polynomial $w_i(s) = \displaystyle\sum_{j=0}^{m_i} w_{i,j} B^{m_i}_j(s)$ requires $\mathcal{O}(m_i^3)$ operations. However, for relatively low degree rational curves, the cost of this root-finding step is minimal and the degree of the component rational curves is often taken to be constant in applications.

\subsubsection{Rational Intermediate Quadrature}
\label{sec:rat_intermediate}
Once the rational poles, $\{p_{i,j}\}_{i=1}^{m_i}$ for each $\mathbf{c}_i$ and their $k+3$ multiplicities are known, the remaining step is to calculate an exact quadrature rule for functions with these poles in the parametric space $0 \leq s \leq 1$ of each $\{\mathbf{c}_{i}\}_{i=1}^{n_c}$. Note that for any polynomial portions of the boundary, a simple Gaussian quadrature rule will be sufficient to achieve an exact intermediate quadrature rule. For the rational portions of the boundary, we must use an exact rational quadrature rule. We choose to use a linear-time algorithm developed in~\cite{deckers2017algorithm}. Implementation details are given in Section~\ref{sec:rational_implementation}. The quadrature points and weights from this algorithm can then be substituted for the Gaussian quadrature points and weights in Section~\ref{sec:intermediate}.


\begin{figure}
\begin{adjustbox}{width=.9\linewidth,keepaspectratio,margin=1.5em 0em 1.5em 0em}
\begin{lstlisting}[style=Matlab-editor,numbers=left]
f = @(x,y) getIntegrand();
kDeg=getDegree(f);
Bd=loadShape();
for i=1:getNumCurves(Bd)
  % Compute intermediate quadrature rule
  if use_SpectralPE
    poles=roots(getWeights(Bd(i)))  %2.5.1
    intPoles=repmat(poles,kDeg+3);  %2.4.2
    [intpts intwts]= 
         calcIntQRule(intPoles);    %2.5.3
  else
    [intpts intwts]= calcIntQRule();  %2.1
  end
  
  % Compute antiderivative quadrature rule
  for j=1:length(intpts)
    [Afx,Afy]=Bd{i}(intpts);
    [ADpts, ADwts]=                   %2.2
         calcAntiderivativeQRule([0,Afx]);
    finalptsx(j,:)=ADpts;
    len = length(finalptsx)
    finalptsy(j,:)=repmat(Afy,len,1); 
    finalwts(j,:)=intwts(j)*ADwts;
  end
  quadrules{i}=[finalptsx,
                finalptsy,
                finalwts ];           %2.3
end
\end{lstlisting}
\end{adjustbox}
\caption{Matlab pseudocode for the quadrature algorithms given in Section~\ref{sec:algorithm}. The function \lstinline{calcIntQRule} is the only difference between the \spectral\ algorithm and the \spectralPE\ algorithm. The first uses a typical high-order quadrature rule, such as Gaussian quadrature. The second uses a quadrature rule exact for rational functions with poles given by \lstinline{intPoles}. Line-by-line comments refer to sections of this article.}
%
% \kennyComment{Please add/modify the code with a few explanatory comments, if/where appropriate. Perhaps, with pointers/references to our equation numbers.}
\label{fig:alg_pseudocode}
\end{figure}

 The resulting exact quadrature rule will have  $n_q$ quadrature points:
 \begin{equation}
   n_q = \left\lceil{\frac{k+1}{2}}\right\rceil\sum_{i=1}^{n_c} \left(m_i(k + 3)+1\right),
 \end{equation}
where $n_c$ is the number of component curves, 
       $m_i$ are the degrees of the component curves $\mathbf{c}_i$, 
       and $k$ is the maximal degree of the polynomial integrand.
 Pseudocode for this algorithm is provided in Figure~\ref{fig:alg_pseudocode}.

\begin{figure}
\begin{minipage}{.235\textwidth}
\begin{center}
\includegraphics[width=\linewidth]{l_bracket_holes_orientations_labeled_update}\\
\large{(a)}
\end{center}
\end{minipage}~
\begin{minipage}{.25\textwidth}
\begin{center}\includegraphics[width=\linewidth]{l_bracket_holes_component_curves_labeled}\\
\large{(b)}
\end{center}
\end{minipage}
\caption{An example of a non genus-zero region with $M=4$ boundary loops and $n_c=20$ component curves. In this case, the maximum degree of the component curves is $m=2$. In (a), the boundary curves $\{\Gamma_\alpha\}_{\alpha=1}^4$ and boundary regions $\{\Omega_\alpha\}_{\alpha=1}^4$ are labeled. In (b), the component curves $\{\mathbf{c}_i\}_{i=1}^{n_c}$ are labeled.}
\label{fig:multiple_components}
\end{figure}

\subsection{Implementation Notes}
In this section, we describe the implementation details we used to produce the numerical results in ~Section~\ref{sec:results}. 
\subsubsection{Poles of Rational Curves--Implementation}
\label{sec:conversion}
In the test cases that follow, we consider $\mathbf{c}_i$ to be given in the Bernstein-\bezier\ basis. In order to find the roots of the control weight polynomial, \begin{equation*}
w_i(s) = \displaystyle\sum_{j=0}^{m_i} w_{i,j} B^{m_i}_j(s),
\end{equation*} 
we use Matlab's \texttt{roots} command~\cite{MATLAB}, which has an optimized algorithm for finding the eigenvalues of the companion matrix of $w_i(s)$. 
%
However, to use Matlab's \texttt{roots} command, we must convert from the Bernstein-\bezier\ basis to the monomial basis, which is an ill-conditioned basis conversion for high-degree polynomials, as discussed in~\cite{farouki1988algorithms}. The condition number of the conversion matrix is generally on the order of $10^{\frac{m}{2}}$, where $m$ is the degree of the polynomial. Approximately $\frac{m}{2}$ digits of precision are therefore lost in this conversion. The conversion matrix from the monomial basis to the Bernstein-\bezier\ basis is defined as
\begin{equation*}
MB_{i,j} = 
\begin{cases}\frac{\binom{n-k+1}{j-k}}{\binom{n}{j-1}} &\text{ for } j\geq k\\
0 &\text{ otherwise, }
\end{cases}
\end{equation*}
and the conversion from the Bernstein-\bezier\ basis to the monomial basis is defined as 
\begin{equation*}
BM_{i,j} = \begin{cases} 
(-1)^{j-k} \binom{n}{j-1} \binom{j-1}{k-1} & \text{ for } j\geq k\\
0 &\text{ otherwise, }
\end{cases}
\end{equation*}
where $BM_{i,j}$ denotes the entry in the $i$-th row and $j$-th column of the matrix. An optimal implementation would instead find roots in the original input basis to avoid basis conversion stability issues. 

\subsubsection{Green's Theorem--Implementation}
\label{sec:green_implement}
The choice of $C$ in the antiderivative computation in Equation~$\eqref{eq:antiderivative}$ affects the locations of the resulting quadrature points. If the $C$ is taken to be very far from the domain of interest, it can affect the floating point stability of the resulting computations, since the antiderivative integrals can become very large in magnitude. In order to keep the quadrature points close to the original domain, we choose $C$ to be the minimum y-component of any control point making up the curves in the boundary loop, $\Gamma$. That is, we choose
\begin{equation*}
C= \min_{i,j} y_{i,j}.
\end{equation*}  
The Gaussian quadrature points used to evaluate the integral in Equation~$\eqref{eq:antiderivative}$ will therefore always lie between the intermediate quadrature point $y$ and the smallest control point of the boundary loop $\Gamma$. Since the points $y$ always lie on the component curves, the quadrature points from the full algorithm will always lie within the bounding box of the control points. 

\subsubsection{Rational Intermediate Quadrature--Implementation}
\label{sec:rational_implementation}
To compute the intermediate quadrature rule for the modification to achieve polynomial exactness in Section~\ref{sec:rat_intermediate}, we use a method developed in \cite{deckers2017algorithm}. The method generates $m+1$ quadrature points when $m$ (possibly non-unique) poles are specified in linear time with respect to the number of poles $m$. The algorithm also ensures a degree of polynomial exactness beyond the default rational exactness. If $m$ poles are specified but $m+l$ quadrature points are requested, the algorithm will be exact for rational functions with the $m$ poles as well as for (one-dimensional) polynomial functions up to degree $l$. Convergence of the \spectralPE\ for arbitrary functions is achieved by increasing this $l$ parameter past that required by the degree of polynomial exactness $k$, for example in Figure~\ref{fig:nonpolynomial_results}.

The algorithm can be used to compute exact quadrature rules on any real interval for any class of rational functions with arbitrary poles outside of the domain of integration (in this case, the unit interval). It is well known that if all of the coefficients of a polynomial in the Bernstein-\bezier\ basis are of the same sign, then the polynomial has no roots within the unit interval \cite{farin2002curves}. Therefore, as long as all of the control weights $w_{i,j}$ in all of the component curves $\mathbf{c}_i$ are positive (a common situation in most applications), the quadrature scheme given in \cite{deckers2017algorithm} is theoretically valid.


\subsection{Remark: Location of Quadrature Points}
As can be seen in Figure~\ref{fig:quadrature_points_circle}, the quadrature points do not, in general, lie within the integration region $\Omega$. However, the quadrature points in our scheme are always contained within the bounding box of the component curves, $\tilde{\Omega}$. 
%
It is sometimes desirable that the locations of the quadrature points be contained within the boundaries of the quadrature region $\Omega$, particularly when dealing with potentially non-analytic integrands. If the original domain is convex, the locations of the quadrature points can be guaranteed to lie within the domain of integration using an appropriate choice of $C$ and a rotation of the coordinate system (see \cite{santin2011algebraic} for implementation details). If the domain is non-convex, a moment-fitting approach could be combined with our algorithm to compute a quadrature rule with only interior quadrature points \cite{thiagarajan2018shape, taber2018moment}. We briefly introduce moment-fitting and describe how it could be used with our method in \ref{app:momentFitting}.

    
\subsection{Remark: Multiple Components}
In some cases, the region of interest may not be genus-zero (i.e., it may have holes or disconnected components), see, for example, the region in Figure~\ref{fig:multiple_components}. In this case, there are multiple boundary loops $\partial \Omega = \{\Gamma_\alpha\}_{\alpha=1}^M$, each of which bounds a genus-zero domain $\Omega_\alpha$. The original domain $\Omega$ is then a finite Boolean (union, intersection, and subtraction) combination of the component genus-zero domains $\Omega_\alpha$. As long as the orientations of each of the boundary curves $\Gamma_\alpha$ are given, the algorithm as stated transfers seamlessly, since it treats each of the component curves $\mathbf{c}_i$ independently. In this case, the integral over $\Omega$ can  be thought of as the signed sum of the integrals over each $\Omega_\alpha$: $\iint_\Omega f(x,y) dxdy = \sum_{\alpha=1}^N s(\alpha) \iint_{\Omega_\alpha} f(x,y) dxdy$, where the indicator function $s(\alpha)$ can be sorted out according to the orientations of the boundary curves:
\begin{equation*}
s(\alpha) = \begin{cases} 1 & \text{ if $\Gamma_\alpha$ is counter-clockwise oriented}\\
-1 & \text{ if $\Gamma_\alpha$ is clockwise oriented}.
\end{cases}
\end{equation*} Our aforementioned algorithm is then applied to each integral individually.



